Stochastic Physics-Informed Neural Networks on Lie Groups for Learning Underwater Vehicle Dynamics

Accurate models of underwater vehicle motion are needed for autonomous execution of marine tasks like infrastructure inspection and scientific sampling. However, such motion is challenging to characterize using traditional physics-based methods. This paper presents a novel data-driven framework for learning stochastic underwater vehicle dynamics. Using Euler-Poincar\'e dynamics and the geometry of Lie groups, we develop a stochastic physics-informed neural network architecture that respects the physical and geometric constraints of underwater vehicles. Our approach leverages structure-preserving stochastic integration and builds upon moment matching and finite dimensional matching to ensure geometrically-consistent training. We evaluate our approach in simulation and on an underwater vehicle navigating dock pylons in a harbor environment. The results demonstrate that our method learns accurate and robust dynamics models, enabling safe model-based control in challenging marine environments.

==> sections/background/uncertainty.tex <==
\subsection{Stochastic Processes on Lie Groups}

Standard treatment of uncertainty in rigid-body systems assumes Euclidean state spaces with additive Gaussian noise. However, additive noise does not accurately represent uncertainty in systems whose states evolve on Lie groups, because Lie groups are not vector spaces. Instead, uncertainty can be represented using the concentrated Gaussian distribution for Lie groups \cite{jayaraman2023lie, chirikjian2012stochastic, ye2025uncertainty, ge2024geometric}. Concentrated Gaussian distributions leverage the observation that Lie algebras are vector spaces. This property allows additive uncertainty to be defined in the Lie algebra, where Euclidean probability models apply. The exponential map then projects the noise onto the group, inducing a distribution.

Formally, define a random variable on the Lie group $G$ as
%
\begin{equation}
    \fiber(\randeuclid) = \mu \exp(\randeuclid),~\randeuclid \sim \gaussian,
\end{equation}
%
where $\randeuclid$ is a random variable associated with the Euclidean normal distribution. The corresponding unimodal probability density function $f(\fiber)$ is defined as,
%
\begin{equation}
\label{eq:concentrated-gaussian}
    f(\fiber) =\frac{1}{(2\pi)^3|\det \Sigma|^\frac{1}{2}}\exp\left(-\frac{1}{2}\|\derep{\log(\inv{\mu} \fiber)}\|_{\inv{\Sigma}}\right),
\end{equation}
%
where the group theoretic mean $\mu \in G$ is,
%
\begin{equation}
    \int_G \derep{(\log(\inv{\mu} \fiber)}f(\fiber)\,\mathrm{d}\fiber = \mathbf{0},
\end{equation}
%
and the covariance $\Sigma$ about $\mu$ satisfies,
%
\begin{equation}
    \Sigma = \int_G \derep{\log(\inv{\mu} \fiber)}\transpose{\derep{\log(\inv{\mu} \fiber)}}f(\fiber)\,\mathrm{d}\fiber.
\end{equation}
%
$f(g)$ is said to be concentrated when $\|\Sigma\|_2 \ll 1$, which ensures that the global topological properties of the group do not affect the distribution. The reader is referred to the following textbook for a more detailed exposition of stochastic modeling on Lie groups \cite{chirikjian2012stochastic}.

==> sections/method/implementation.tex <==
\subsection{Implementation Details}

We implement all neural networks as multi-layer perceptrons (MLPs) using \texttt{JAX} \cite{jax2018github} and \texttt{Equinox} \cite{kidger2021on}. The hydrodynamic coefficients, including rigid-body and fluid-added mass $M_\neuralparams$, viscous drag $\viscousdrag_\neuralparams$, and fluid drag $\fluiddrag_\neuralparams$ are modeled as
%
\begin{subequations}
\label{eq:hydrodynamic-networks}
\begin{align}
    % option 1:
    \net_M &: \SEthree \rightarrow \Spdsix, & \fiber &\mapsto M_\neuralparams \\
    \net_{\viscousdrag} &: \sethree \rightarrow \Spdsix, & \fibercirc &\mapsto \viscousdrag_\neuralparams \\
    \net_{\fluiddrag} &: \sethree \rightarrow \Spdsix, & \fibercirc &\mapsto \fluiddrag_\neuralparams
    % option 2:
    % \net_M &: \SEthree \rightarrow \Spdsix \\
    % &: \fiber \mapsto M_\neuralparams \\[3pt]
    % \net_{\viscousdrag} &: \sethree \rightarrow \Spdsix \\
    % &: \fibercirc \mapsto \viscousdrag_\neuralparams \\[3pt]
    % \net_{\fluiddrag} &: \sethree \rightarrow \Spdsix \\
    % &: \fibercirc \mapsto \fluiddrag_\neuralparams
    % old:
    % M_\neuralparams &: \SEthree \rightarrow \Spdsix \\
    % \viscousdrag_\neuralparams &: \euclid^6 \rightarrow \Spdsix \\
    % \fluiddrag_\neuralparams &: \euclid^6 \rightarrow \Spdsix
\end{align}    
\end{subequations}
%
where $\Spdsix$ denotes the manifold of $6 \times 6$ symmetric positive-definite (SPD) matrices. Positive-definiteness is achieved by applying a positive-valued nonlinear function (e.g., softplus, $\exp$, etc.) to the eigenvalues of the $\euclid^{6 \times 6}$ matrices predicted by an MLP. 

We model the learned potential energy as
%
\begin{equation}
    \net_\potentialenergy : \SEthree \rightarrow \euclid, \qquad \fiber \mapsto \lambda\,\text{tanh}\left(\text{MLP}_{\neuralparams_\potentialenergy}(\fiber)\right)
    % \potentialenergy_\neuralparams &: \SEthree \rightarrow \euclid \\
    % &: \fiber \mapsto \lambda\,\text{tanh}\left(\text{MLP}_\neuralparams(\fiber)\right).
\end{equation}
%
The learned scalar $\lambda \in \euclid$ (part of $\neuralparams$) and final tanh nonlinearity are applied to the MLP output to constrain the rate of change in the hidden state \cite{kidger2021on}. We found that without these constraints, the optimizer tends to over-rely on the potential energy term to minimize the loss and implicitly regularizes the hydrodynamic coefficient networks \eqref{eq:hydrodynamic-networks}.

The approximated diffusion $\neuralcovdiffusion$ is implemented as
%
\begin{equation}
    \net_\covdiffusion : \SEthree \times \sethree \rightarrow \text{Diag}_+^6, \qquad
    \left( \fiber, \fibercirc \right) \mapsto \neuralcovdiffusion
    % \neuralcovdiffusion : \SEthree \times \euclid^6 \rightarrow \text{Diag}_+^6,
\end{equation}
%
where we restrict $\neuralcovdiffusion$ to a $6 \times 6$ diagonal matrix to simplify loss calculations, and we apply a positive-valued nonlinear function to the model outputs.

